Multi-level Protein Representation Learning for Blind Mutational Effect Prediction

Directed evolution plays an indispensable role in protein engineering that revises existing protein sequences to attain new or enhanced functions. Accurately predicting the effects of protein variants necessitates an in-depth understanding of protein structure and function. Although large self-supervised language models have demonstrated remarkable performance in zero-shot inference using only protein sequences, these models inherently do not interpret the spatial characteristics of protein structures, which are crucial for comprehending protein folding stability and internal molecular interactions. This paper introduces a novel pre-training framework that cascades sequential and geometric analyzers for protein primary and tertiary structures. It guides mutational directions toward desired traits by simulating natural selection on wild-type proteins and evaluates the effects of variants based on their fitness to perform the function. We assess the proposed approach using a public database and two new databases for a variety of variant effect prediction tasks, which encompass a diverse set of proteins and assays from different taxa. The prediction results achieve state-of-the-art performance over other zero-shot learning methods for both single-site mutations and deep mutations.

==> checklist.tex <==
\newpage
\section*{Checklist}
% \url{https://neurips.cc/public/guides/PaperChecklist}

\begin{enumerate}
    \item \textbf{Claims}: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope? 
      \answerYes{We state clearly the scope and contribution of both communities of protein engineering and computer science in the abstract and introduction.}
    \item \textbf{Code Of Ethics}: Have you read the NeurIPS Code of Ethics (\url{https://neurips.cc/public/EthicsGuideline}s) and ensured that your research conforms to it?
      \answerYes{The general ethical conduct has been carefully gone through to make sure the listed concerns are avoided or not applicable in this research. }
    \item \textbf{Broader Impacts}: If appropriate for the scope and focus of your paper, did you discuss potential negative societal impacts of your work?     
      \answerYes{See Section~\ref{sec:discussion}.}
    \item \textbf{Limitations}: Did you describe the limitations of your work? You are encouraged to create a separate Limitations section in your paper. 
      \answerYes{See Section~\ref{sec:discussion}.}
    \item \textbf{Theory}: If you are including theoretical results, did you state the full set of assumptions of all theoretical results, and did you include complete proofs of all theoretical results? 
      \answerNA{}
    \item \textbf{Experiments}: If you ran experiments, did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
      \answerYes{Implementation details (pre-processing, model configuration, code availability, etc) are listed in Section~\ref{sec:experiment}, with additional information regarding the new benchmark and competitive methods supplemented in Appendix~\ref{sec:app:Tm_DDG} and Appendix~\ref{sec:app:baselineImplementation}, respectively. }
    \item \textbf{Training Details}: If you ran experiments, did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
      \answerYes{We disclose full implementation details of our model in Section~\ref{sec:experiment}. Baseline methods are pre-trained by their authors, which requires no further supervision or learning procedures.}
    \item \textbf{Error Bars}: If you ran experiments, did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
      \answerNA{Measurements used in this work return fixed results on a determined model, and a pre-trained model barely trains a set of models under the same dataset or hyper-parameter settings.}
    \item \textbf{Compute}: Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
      \answerYes{Details for the running machine are provided at the beginning of Section~\ref{sec:experiment}}.
    \item \textbf{Reproducibility}: If the contribution is a dataset or model, what steps did you take to make your results reproducible or verifiable?
      \answerYes{We provide the hyper-parameter settings in the main text and upload the main algorithm as well as the benchmark dataset in the anonymous repository.}
    \item \textbf{Safeguards}: Do you have safeguards in place for responsible release of models with a high risk for misuse (e.g., pretrained language models)? 
      \answerNA{We did not study generative models.}
    \item \textbf{Licenses}: If you are using existing assets (e.g., code, data, models), did you cite the creators and respect the license and terms of use? 
      \answerYes{We cite all the papers for baseline methods and the one existing benchmark (ProteinGym). The reproduced results are based on the latest release on their GitHub repositories, which we attached URLs in Appendix~\ref{sec:app:baselineImplementation}.}
    \item \textbf{Assets}: If you are releasing new assets, did you document them and provide these details alongside the assets?
      \answerYes{We revealed the full detail of the new benchmark dataset in Appendix~\ref{sec:app:Tm_DDG} and released it in our anonymous repository.}
    \item \textbf{Human Subjects}: If you used crowdsourcing or conducted research with human subjects, did you include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
      \answerNA{we did not conduct research with human subjects.}
    \item \textbf{IRB Approvals}: Did you describe any potential participant risks and obtain Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your institution), if applicable?
      \answerNA{we did not conduct research with human subjects.}


\end{enumerate}
